Search for new phenomena in final states with an energetic jet and large missing transverse momentum in pp collisions at $\sqrt{s}=8$ TeV with the ATLAS detector

Results of a search for new phenomena in final states with an energetic jet and large missing transverse momentum are reported. The search uses 20.3 fb$^{-1}$ of $\sqrt{s}=8$ TeV data collected in 2012 with the ATLAS detector at the LHC. Events are required to have at least one jet with $p_T > 120$ GeV and no leptons. Nine signal regions are considered with increasing missing transverse momentum requirements between $E_T^{miss} > 150$ GeV and $E_T^{miss} > 700$ GeV. Good agreement is observed between the number of events in data and Standard Model expectations. The results are translated into exclusion limits on models with large extra spatial dimensions, pair production of weakly interacting dark matter candidates, and production of very light gravitinos in a gauge-mediated supersymmetric model. In addition, limits on the production of an invisibly decaying Higgs-like boson leading to similar topologies in the final state are presented.

==> wimps_sys.tex <==

The ATLAS cross section limits are converted into limits on the pair
production of WIMPs in the EFT framework. For each EFT operator, the
limits are extracted from those signal regions that exhibit the best
expected sensitivity: these are SR4 for C1, SR7 for C5, D1, D5, D11,
and SR9 for D9. The corresponding 95\% CL \MS{} limits are plotted
versus the DM particle mass ($m_\chi$) in
Figure~\ref{fig:wimp:ms} for a representative set of three operators.

To derive these lower limits on \MS{}, the experimental systematic
uncertainties due to the jet energy scale, the jet energy resolution
and the reconstruction of \MET{} are considered as a single correlated
uncertainty of both the signal and background events. Other
experimental sources of systematic uncertainty, such as the beam
energy~\cite{Wenninger:1546734} and luminosity, enter the limit
calculation only as uncertainty of the signal events.

The theoretical uncertainties considered are related to the parton
matching scale used for the {MADGRAPH5} signal samples, to the
factorization and renormalization scales, and to the PDF. In all
cases, experimental or theoretical systematic uncertainties that
affect the acceptance, that is, the shape of the \met\ distribution in
the signal region, are taken into account when deriving the actual
$CL_s$ limits on \MS{}, those uncertainties affecting the overall
cross section only are displayed as error band around the expected
limit (see Fig.~\ref{fig:wimp:ms} below). 

The beam energy uncertainty is considered by simulating WIMP samples
with the lower and upper allowed values given in
Ref.~\cite{Wenninger:1546734}. The parton matching scale uncertainty
is determined by varying the parton \pt{} thresholds for the WIMP
sample generation. The ISR/FSR uncertainty is evaluated by comparing
simulated samples with enhanced and suppressed parton emission (using
$\alpha_{\rm s}(2\pt)$ and $\alpha_{\rm s}(\pt/2)$, respectively) to the nominal
ones generated with {Perugia2012} tunes~\cite{perugia} 370, 371
and 372 in {Pythia}. The PDF uncertainty is determined by
comparing the {MSTW2008LO}, {CTEQ6M} and {NNPDF21LO} PDF
sets. And finally the factorization and renormalization scales are
varied simultaneously up and down by a factor of two in {\tt
  MADGRAPH5}.

In summary, the uncertainties and their values considered for the
acceptance and overall cross section are:
\begin{itemize}
  \item \textbf{Acceptance:}
    \begin{itemize}
    \item Beam energy (3\%)
    \item Renormalization and factorization scales (3\%)
    \item Parton matching scale (5\%)
    \item Luminosity (2.8\%)
    \item Jet energy scale, resolution, \met\ (1--10\%, depending on
      the operator and the signal region)
    \item PDF (5--29\%, depending on the operator and WIMP mass)
    \end{itemize}
  \item \textbf{Cross section:}
    \begin{itemize}
      \item Renormalization and factorization scales (2--17\% for D1,
        D5, D9 and 40--46\% for C5 and D11)
      \item Beam energy (2--9\%)
      \item PDF (increasing with WIMP mass, 19--70\% for C5, D11, D1,
        5--36\% for D5, D9
    \end{itemize}
\end{itemize}
Other uncertainties, like those related to the hadronic showering
($\alpha_{\rm s}$ values and ISR/FSR tunes) or the trigger efficiency and
jet cleaning procedure are below the 1\% level and ignored as they are
negligible.

